Voyageur: An Experiential Travel Search Engine

We describe Voyageur, which is an application of experiential search to the domain of travel. Unlike traditional search engines for online services, experiential search focuses on the experiential aspects of the service under consideration. In particular, Voyageur needs to handle queries for subjective aspects of the service (e.g., quiet hotel, friendly staff) and combine these with objective attributes, such as price and location. Voyageur also highlights interesting facts and tips about the services the user is considering to provide them with further insights into their choices.

==> demo.tex <==
\section{Demo of \system} \label{sec:demo}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\textwidth]{hotel_page.pdf}
%     \caption{A screen shot of \system.}
%     \label{fig:screenshot}
% \end{figure*}

==> related.tex <==
\section{Related work} \label{sec:related}
